TensorLib: A Spatial Accelerator Generation Framework for Tensor Algebra

Tensor algebra finds applications in various domains, and these applications, especially when accelerated on spatial hardware accelerators, can deliver high performance and low power. Spatial hardware accelerator exhibits complex design space. Prior approaches based on manual implementation lead to low programming productivity, rendering thorough design space exploration impossible. In this paper, we propose TensorLib, a framework for generating spatial hardware accelerator for tensor algebra applications. TensorLib is motivated by the observation that, different dataflows share common hardware modules, which can be reused across different designs. To build such a framework, TensorLib first uses Space-Time Transformation to explore different dataflows, which can compactly represent the hardware dataflow using a simple transformation matrix. Next, we identify the common structures of different dataflows and build parameterized hardware module templates with Chisel. Our generation framework can select the needed hardware modules for each dataflow, connect the modules using a specified interconnection pattern, and automatically generate the complete hardware accelerator design. TensorLib remarkably improves the productivity for the development and optimization of spatial hardware architecture, providing a rich design space with trade-offs in performance, area, and power. Experiments show that TensorLib can automatically generate hardware designs with different dataflows and achieve 21\% performance improvement on FPGA compared to the state-of-the-arts.

==> background.tex <==
\section{Background}

\subsection{Systolic Array}
Systolic array defines an operational principle of specialized accelerator for dense tensor algorithms. A common systolic array is composed of a 2D meshgrid of PEs. Each data element transfer from one PE to its adjacent PE every cycle, and follows a fixed direction. The common feature of systolic array can be derived from two folds. First, all PEs have the same hardware component. Second, data communication network is always the combination of vertical interconnection, horizontal interconnection and diagonal interconnection between adjacent PEs. 

% The behavior of every PEs are similar, and all PEs are controlled by a global synchronous clock.
% is a highly flexible architecture which supports different tensor algorithms with multiple dataflows and other configurations. 
% In systolic architectures, each PE only transfer data with its adjacent PEs, and only the PEs at the edge can transfer data with outer system. The systolic array architecture overcomes the problem of low memory transaction speed by converting global memory transactions into high-speed local communication between adjacent PEs. 

\subsection{Hardware Design Language}
Traditional hardware-description languages (HDLs), Verilog and VHDL lack the high-level abstraction of systolic array features, which is a time-consuming approach and requires prior experience. High Level Synthesis (HLS) improves the productivity and shows higher specification in the language. However, HLS uses imperative programming which limits its modularity, and often leads to more resource consumption. 

Chisel\cite{chisel} is a hardware description language based on Scala language. It brings the features of software programming to the area of hardware construction, such as standard hardware library, object-oriented programming, type-generic and meta-programming features. In this paper, we build a systolic array generator with parameterized and modular templates written in Chisel. 
% Chisel lo
% With the help of Chisel, hardware programmers can improve their productivity by using easy abstractions such as standard hardware library, object-oriented programming, type-generic and meta-programming features. Chisel has powered many influential projects, such as Rocket Chip Generator\cite{rocketchip}, the Spatial Language\cite{Spatial}, and the ACED DSP library\cite{aced}. \cite{compare} shows that well-optimized Chisel-based implementation of hardware can achieve same performance as low-level HDLs, and requires less LOCs (line of codes).
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.92\textwidth]{figs/bothflow_v4.pdf}
%     \caption{Systolic Dataflow for Matrix Multiplication}\label{fig:dataflow}
% \end{figure*}

==> tab.tex <==
\begin{table}[t]
    \small
    \centering
    \caption{Morphling area and power breakdown}\label{tab:breakdown}
    \begin{tabular}{ccc} 
    \toprule[2pt]
                            & \textbf{Configuration}                                                      & \textbf{Description}   \\ 
    \hline
    \multirow{5}{*}{PE Level}     & SIMD Compute Unit Size    & Each PE performs a SIMD vectorized MAC operation.\\ With both operands vectorized, the operation becomes an outer-product.  \\ 
    \cline{2-3}
                            & Precision \& Bitwidth                                                           & Data percision or bitwidth, can be int8, int16, float16, float32, etc.     \\ 
    \cline{2-3}
                            & FU                                                             & 0.215           \\ 
    \cline{2-3}
                            & Memory                                                         & 0.239 \\ 
    \cline{2-3}
                            & Total                                                          & 0.738 \\ 
    \hline
    \multirow{3}{*}{Systolic-Array Level} & AL                                                             &        0.089            \\ 
    \cline{2-3}
                            & Memory                                                         &           0.119       \\ 
    \cline{2-3}
                            & Total                                                          &    d   \\ 
    \bottomrule[2pt]
    \end{tabular}
    \end{table}
